Multilingual Previously Fact-Checked Claim Retrieval

Fact-checkers are often hampered by the sheer amount of online content that needs to be fact-checked. NLP can help them by retrieving already existing fact-checks relevant to the content being investigated. This paper introduces a new multilingual dataset -- MultiClaim -- for previously fact-checked claim retrieval. We collected 28k posts in 27 languages from social media, 206k fact-checks in 39 languages written by professional fact-checkers, as well as 31k connections between these two groups. This is the most extensive and the most linguistically diverse dataset of this kind to date. We evaluated how different unsupervised methods fare on this dataset and its various dimensions. We show that evaluating such a diverse dataset has its complexities and proper care needs to be taken before interpreting the results. We also evaluated a supervised fine-tuning approach, improving upon the unsupervised method significantly.

==> related-work-notes.tex <==
% TODO (Timo Hromadka) - 
% % !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
% % !!!!!!!!    TODO     !!!!!!!!!!!!
% % !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
% Key things to mention as themes across this section:
% - only focusong in claim matching vs. full social media post matching (noisier)
% - multinguality

% Section split as follows:
% 1. Previously fact checked claim detection's similar fields, and how it hasnt been studied too extensively
% 2. Checkthat lab introduction
% 3. Overview of baseline methods (including CheckThat datasets)
%     - checkthat teams (generally initial retrieve, semantic similarity with cosine, and rerank)
        
%     1. use of reranking
%     2. use of sbert
%     3. use of snopes or politifact
% 4. Overview of other atypical methods
%     - other methods (graphical, context based, feature based, etc)
% 5. overview of current datasets
%     - datasets (snopes, politifact)
%     - some have only fact check claims 
%         - Liar Liar (12.8k claims from Politifact)
%         - MultiFCC (38k claims from 26 FC organizations)
%         - Truth of Various Shades (10k claims)
% 6. talk about limitations of works
% 7. outline what our paper will bring to community (but dont repeat what was said in introduction)



% ===================================================================================
% ========================          START OF TEXT            ========================
% ===================================================================================
% Previously Fact-Checked Claim Detection was namely introduced in CLEF's CheckThat! competition in 2020 \citep{checkthat_2020} and subsequently continued in 2021 \citep{checkthat_2021} and 2022 \citep{checkthat_2022} (See Table~\ref{table:pfcd_datasets}). Typically, teams working with their datasets utilized a three step pipeline of 1) pre-processing; 2) similarity retrieval with BM25~\citep{bm25_2009}, Elastic Search, TF-IDF, and/or fine-tuned Sentence-BERT transformers~\citep{sbert_2019}; and 3) re-ranking using two or more methods from step 2~\citep{buster_checkthat_2020, checksquare_checkthat_2020, sheffield_checkthat_2020, ubet_checkthat_2020, unipinle_checkthat_2020, aschern_checkthat_2021, dips_checkthat_2021, shaar-etal-2020-known, simba_checkthat_2022, fraunhofer_checkthat_2022, mansour_did_2022, beasku_checkthat_2021}. Some teams incorporated a neural re-ranker~\citep{nlpiruned_checkthat_2020, nlytics_checkthat_2021, bigir_checkthat_2021, riet_checkthat_2022}. Other approaches include using a fine-tuned \texttt{ROUGE}-guided~\citep{rouge_2004} transformer, pattern-sentence graph matching, key sentence extraction, and score-weighted aggregation \citep{Sheng_2021}, abstractive summarization with seq2seq models and decoding strategies~\citep{bhatnagar_abstractive_summarization_2022}, reverse image search for additional semantic context~\citep{mansour_did_2022}, or ResNet~\citep{resnet_2015}, GloVe \citep{glove_2014}, and ELMo~\citep{elmo_2018} features fed into a CNN~\citep{vo_lee_facts}. 


% % =====================================================================
% % ========================= OLD VERSION ===============================
% % =====================================================================
% Previously fact-checked claim detection (PFCD) has been recognized as a crucial and necessary learning-to-rank task within a holistic end-to-end fact-checking pipeline \citep{hassan_claimbuster_2017}. Whilst there exist many analogous and helper tasks related to PFCD, such as Sentence Text Similarity [ref], Paraphrase Detection [ref], or Content Matching [ref], the task has only been given attention in the last couple of years, with its recognition namely attributed to CLEF's CheckThat! competition. The PFCD task was introduced in 2020 \citep{checkthat_2020} and subsequently continued in 2021 \citep{checkthat_2021} and 2022 \citep{checkthat_2022}. The competition accompanied the release of three datasets (two English, one Arabic) collected from Politifact\footnote{\url{http://www.politifact.com/}} and Snopes\footnote{\url{http://www.snopes.com/}} containing claims and their corresponding fact-checking (FC) articles.

% Typically, teams working with these datasets utilized a three step pipeline of 1) pre-processing; 2) similarity retrieval with BM25~\citep{bm25_2009}, Elastic Search, TF-IDF, or fine-tuned Sentence-BERT transformers~\citep{sbert_2019}; and 3) re-ranking using two or more methods from step 2~\citep{buster_checkthat_2020, checksquare_checkthat_2020, sheffield_checkthat_2020, ubet_checkthat_2020, unipinle_checkthat_2020, aschern_checkthat_2021, dips_checkthat_2021, shaar-etal-2020-known, simba_checkthat_2022, fraunhofer_checkthat_2022, mansour_did_2022, beasku_checkthat_2021}. Some teams incorporated a neural re-ranker~\citep{nlpiruned_checkthat_2020, nlytics_checkthat_2021, bigir_checkthat_2021, riet_checkthat_2022}. \citet{crowdchecked_2022} constructed a custom crawled dataset, along with CheckThat! fact checks, to investigate learning from noisy data with self-adaptive training using distant supervision. FC-article ranking was pursued on a Chinese dataset, with claims collected from Chinese Weibo and FC-articles collected from mutliple sources, using a fine-tuned \texttt{ROUGE}-guided~\citep{rouge_2004} transformer, pattern-sentence graph matching, key sentence extraction, and score-weighted aggregation to assess the relevance of a claim to a corpus of FC-articles \citep{Sheng_2021}. 

% It must be recognized that social media posts (SMP) contain highly unstructured and noisy text, and thus provide a more challenging task than standard claim-matching. To denoise SMPs, in particular Indian context tweets, \citet{bhatnagar_abstractive_summarization_2022} experimented with various seq2seq and decoding strategies for abstractive summarization to obtain crisp claims. The generated claims were assessed against Google's \textit{Fact Check Explorer}\footnote{\url{https://toolbox.google.com/factcheck/explorer}} tool, which can naturally only handle clean claims. \citet{mansour_did_2022} utilized the CheckThat! datasets with reverse image search on URLs to extract FC titles for additional semantic context. \citet{vo_lee_facts} utilized a dataset from \citep{vo_learning_2019} to construct tweet to FC-article pairs. Images, if present, in the tweet and FC-article were decoded with ResNet~\citep{resnet_2015}, and text was transformed into features using GloVe \citep{glove_2014}, ELMo~\citep{elmo_2018} and later fed into a CNN. 

% Despite a modest amount of progress on the PFCD learning-to-rank task, there exist only a few SMP to FC-article datasets, none of which are multingual and/or of substantial size. Existing datasets related to our task are summarized in Table~\ref{table:pfcd_datasets}.

% \begin{table}[]
% \centering
% %\setlength{\tabcolsep}{20pt}
% \renewcommand{\arraystretch}{1.6}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{llll}
% \hline
% \hline
% \Large{\textbf{Dataset}}                                                                & \Large{\textbf{Input claims}}       & \Large{\textbf{Verified claims}} & \Large{\textbf{Confirmed pairs}} \\ \hline
% CheckThat! Debates EN \citep{checkthat_2022} & \Large{669}         & \Large{19,250}  & \Large{804}             \\ \hline
% CheckThat! Tweets EN \citep{checkthat_2022} & \Large{1,601}       & \Large{13,835}  & \Large{1,601}            \\ \hline
% CheckThat! Tweets AR \citep{checkthat_2022}   & \Large{908}         & \Large{30,329}  & \Large{1,039}            \\ \hline
% CrowdChecked~\citep{crowdchecked_2022}   & \Large{316,564}     & \Large{10,340}  & \Large{-}               \\ \hline
% \citealp{kazemi_claim_2021}   & \Large{-}     & \Large{-}  & \Large{2,343}               \\ \hline
% COVIDLies \citep{hossain-etal-2020-covidlies}         & \Large{6,761}       & \Large{86}     & \Large{-}               \\ \hline
% IFCN \citep{jiang_categorising_2021}             & \Large{182,000,000} & \Large{10,381}  & \Large{-}               \\ \hline \hline
% Our Dataset             & \Large{28,092}         & \Large{240,000}  & \Large{\textbf{30,000}}             \\ \hline
% \end{tabular}}
% \caption{Existing datasets for Previously Fact Checked Claim Detection. A '-' field indicates an unreleased or non-existant portion of the dataset.}
% \label{table:pfcd_datasets}
% \end{table}

% ... TODO : finalize numbers for our dataset when closer to submission

% \begin{table}[]
% \centering
% %\setlength{\tabcolsep}{20pt}
% \begin{tabular}{llll}
% \hline
% \hline
% \textbf{Dataset}                                                                & \textbf{Input claims}       & \textbf{Verified claims} & \textbf{Confirmed pairs} \\ \hline
% CheckThat! Debates EN \citep{checkthat_2022} & 669         & 19,250  & 804             \\ \hline
% CheckThat! Tweets EN \citep{checkthat_2022} & 1,601       & 13,835  & 1,601            \\ \hline
% CheckThat! Tweets AR \citep{checkthat_2022}   & 908         & 30,329  & 1,039            \\ \hline
% CrowdChecked~\citep{crowdchecked_2022}   & 316,564     & 10,340  & 0               \\ \hline
% \citealp{kazemi_claim_2021}   & -     & -  & 2,343               \\ \hline
% COVIDLies \citep{hossain-etal-2020-covidlies}         & 6,761       & 86     & -               \\ \hline
% IFCN \citep{jiang_categorising_2021}             & 182,000,000 & 10,381  & -              \\ \hline \hline
% Our Dataset             & 24,000         & 240,000  & \textbf{30,000}             \\ \hline
% \end{tabular}}
% \caption{Existing datasets for Previously Fact Checked Claim Detection. A '-' field indicates an unreleased or non-existant portion of the dataset.}
% \label{table:pfcd_datasets}
% \end{table}

% Note that \citep{hossain-etal-2020-covidlies, jiang_categorising_2021, kazemi_claim_2021} include a labelled dataset to be used for a classification task, which poses an analogous PFCD task but is systematically simpler and unfeasible to use when searching through a large corpus of FC articles. Furthermore, \citet{crowdchecked_2022} uses distant supervision to train with noisy data, but does not provide any certainty for confirmed pair deduction in their published \textit{CrowdChecked} dataset. \citet{checkthat_2021} uses already processed claims instead of unstructured SMPs, which is less versatile to real-world scenarios. Some datasets only extract tweets with hashtag keywords pertaining to a specific topic (e.g., \texttt{\#covid-19}), introducing bias by focusing only on a narrow scope of topics \citep{hossain-etal-2020-covidlies, jiang_categorising_2021}. Finally, no existing dataset contains FC-articles from more than just a few FC organizations, nor includes multiple languages. The exception to this is \citealp{kazemi_claim_2021}, which includes 4 kindred South Asian languages as well as English, yet most of their confirmed pairs are only SMP-SMP. 

% Our dataset provides the ground necessary for rigorous and prominent analysis over a multitude of areas, as presented in \ref{main_contributions}. Our contributions aim to advance the field of claim matching, and provide the community with a large-scale dataset for training.

% ========================================================================================



% - standard to checkthat labs
%     % - \citep{mansour_did_2022}
%     % \citep{shaar-etal-2020-known} 
% - novelties + those that match our task
%     % - \citep{jiang_categorising_2021}
%     % - full post
%     % - has their own dataset
%     % - \citep{vo_lee_facts}
%     % - matrices
%     % - OCR like us
%     % - full article
%     % - \citep{Sheng_2021}
%     % - pattern memory bank k nearest neighbor procedure
%     % - \citep{bhatnagar_abstractive_summarization_2022}
%     % - abstractive summarization
%     % - \citep{you_attributed_2020}
%     % - doesnt even look at text, just spatial network and graph attention network
%     % - contextual information regarding URLS and SMP
%     % - %TODO - add this or no?
% - datasets
%     - people dont properly use SMP-FC datasets
%     - \citep{wang_relevant_2018} only claims, stance detection task, custom stance-labeled corpus dataset 
%     - \citep{crowdchecked_2022}
%     - and its limitations \^
%     - \citep{jiang_categorising_2021}
%     - small twitter covid
%     - \citep{checkthat_2020}
%     - \citep{checkthat_2021}
%     - COVIDLies \citep{hossain-etal-2020-covidlies}
%     % - not our task \citep{vo_learning_2019} % {Learning from {Fact}-checkers: {Analysis} and {Generation} of {Fact}-checking {Language}},
% - talk about limitations of work
% - outline what paper will bring to community




% -------------------------------------------------------------------------------------
% --------------                       Too Broad                           ------------
% -------------------------------------------------------------------------------------
% \paragraph{General NLP/CL/IR review}
% Homogenous NLP tasks - Semantic matching, STS, Cross lingual claim matching, duplicate identification, search, textual entailment, paraphrase detection, information retrieval.

% - What is STS/multilingual STS? What is IR/multilingual IR? Importantly, this task most suitably falls into the category of CLCM (Cross Lingual Content Matching), or Entity Matching
%     - whilst there has been a lot of work out there, it generally falls into the same few categories. These main categories include information transfer (high resource to low resource), CL named entity recognition, CL POS tagging, CL QA (lots on this, similar to our task), CL (abstractive) summarization, CL emotion detection, etc. etc. Go over previous cross lingual methods, such as Dictionary approaches, Machine Translation, rule based approaches
%     - Perhaps we can direct readers to a few prominent overview papers, and summarize the advances in recent years. Some such overviews include: TODO!
%     - \citep{limkonchotiwat-etal-2022-cl} % CL-ReLKT: Cross-lingual Language Knowledge Transfer for Multilingual Retrieval Question Answering
%     - TODO: read up on this for the exact architecture, dont understand it fully yet
%     - \citep{chittilla-khalil-2022-huaams} % Combining Translation and Domain Pre-training for Cross-lingual News Article Similarity
%     - uses machine translation and ensemble method (XLMR, XLMR-Pre, XLMR-Aug)
%     - \citep{haim-meirom-bobrowski-2022-unsupervised}
%     - Geometric and Topoligcal Methods to understand structure of sentences uniformly across languages
%     - \citep{agarwal-etal-2022-zero}
% - What is BM25? \citep{robertson_bm25_2009} % The Probabilistic Relevance Framework: BM25 and Beyond
% - What are embeddings? Shortcoming in multilingual settings due to low resource availability. Further details and citations provided in previous report. However, for this paper, this is really not neccessary, and deserves only spare mentioning. Perhaps one sentence for them all.
%     - \citep{sbert_2019} % Sentence-BERT: Sentence Embeddings using Siamese BERT-Networks
%     -- SBert - what is it and how it generalizes embeddings into comprehensible vector embeddings
%     - GloVe (https://nlp.stanford.edu/pubs/glove.pdf) % GloVe: Global Vectors for Word Representation
%     - CoVe, 
%     - LASER,
%     - LaBSE, 
%     - mUSE, 
%     - mBERT,
%     - XLM Roberta, 
%     - \citep{kazemi-etal-2021-claim}, % Claim Matching Beyond English to Scale Global Fact-Checking
%     - knowledge distillation, using teacher model (high-resource language) to train student model (low-resource language)
%     - not too relevant, but worth at least a sentence to denote multingual knowledge transfer    
% % TODO: Keep anything mentioned above? 
% % where should multingual embeddings go? What about BM25? Or are these already too established to have any mention whatsoever?



% ======================================================
% =========== SOURCES FOR PREVFCDETECT =================
% ======================================================

% \paragraph{Domain Specific Fake News Detection/Previously Fact Checked Claim Detection}
% \citep{shaar-etal-2020-known}, % That is a Known Lie: Detecting Previously Fact-Checked Claims
% *only structured text
% - Snopes and Politifact
% - only uses structured, verified claims. We use (unstructured) Social Media posts (a harder problem). Note the difference.
% - LM embeddings + BM25 w/ Rank Aggregation
% - Standard pipeline, but provides decent insight
% - uses entire fact check article, not just claim
% - \textbf{does exactly our task}
% \citep{shaar_assisting_2021}, % Assisting the Human Fact-Checkers: Detecting All Previously Fact-Checked Claims in a Document
% - top claim extraction
% - Instead of feeding a complete piece of text (SMP), this proposed architecture feeds in (unstructured) text, and on the output is a list of its top verifiable claimed sentences along with their respective evidence from the fact check database
% - we do not do this step, and instead always encode the text as whole, or as a sliding window
% \citep{shaar_overview_2021}, % Overview of CheckThat! 2020: Automatic Identification and Verification of Claims in Social Media
% - Task 2 (Given a check-worthy claim and a dataset of verified claims, rank the verified claims, so that those that verify the input claim (or a sub-claim in it) are ranked on top of the list [82]
% - "To construct our verified claims collection, we selected 5,921 Arabic claims from AraFacts [28], and 24,408 English claims from ClaimsKG [29], which we translated to Arabic using the Google translate API." (For Arabic Dataset)
% - Snopes (for English Dataset)

% - Teams
% 1. BusterAI
%     - standard pipeline
% 2. UNIPI-NLE
%     - standard pipeline
% 3. UB-ET
%     - standard pipeline
% 4. NLP IR UNED
%     - USE with neural network using cos sim
%     - neural addition
% 5. UOSheffield
%     - standard pipeline
% 6. trueman and elecdlnlp
%     - standard pipeline
% 7. Checksquare
%     - standard pipeine
%     - KDsearch didnot improve, so dont bother adding it into the paper
% 8. iit
%     - standard pipeline
    
% \citep{nakov_clef_2021} % Overview of the CLEF--2021 CheckThat! Lab on Detecting Check-Worthy Claims, Previously Fact-Checked Claims, and Fake News
% - same as shaar\_overview\_2021 but new version.
% - from what i understood, same dataset as last years (claimskg + snopes)
% - dataset available here (https://sites.google.com/view/clef2021-checkthat/)
% - all teams improved over Elastic Search (BM25) baseline. Typically used bm25 + embeddings + reranking in some format. This captures both lexical and semantical features. Teams and summaries are outlined below:
%     - \textbf{Aschern} \citep{aschern_checkthat_2021} % Aschern at CheckThat! 2021: Lambda-Calculus of Fact-Checked Claims
%     - standard pipeline
%     - TFIDF + SBERT fine-tuned on task data + LambdaMART (features are relevances scores and ranks from sBERT and TFIDF)
%     - \textbf{NLytics} \citep{nlytics_checkthat_2021} % NLytics at CheckThat! 2021: Multi-class fake news detection of news articles and domain identification with RoBERTa - a baseline model
%     - used RoBERTa with regression function in final layer to transform the problem into a ranking task
%     - neural addition
%     - \textbf{DIPS} \citep{dips_checkthat_2021} % DIPS at CheckThat! 2021: Verified Claim Retrieval
%     - SBERT cossims + inputting sorted list of cossims into neural layer + RankSVM to obtain final results
%     - \textbf{bigIR} (Arabic Dataset) \citep{bigir_checkthat_2021}
%     - used ArabERT transformer with 2 neural layers on top  to predict relevance score for given tweet-VerClaim pair.
%     - neural addition

% \citep{shaar-etal-2022-role}, % The Role of Context in Detecting Previously Fact-Checked Claims
% - *novelty
% - "We did this by modeling the local context, the global context, as well as by means of co-reference resolution, and reasoning over the target text using Transformer-XH"
% - modelled local context, global context, and co-reference resolution
% - constructs features from surrounding context (local context)
% - Graph based transformer approach on top-100 bm25 results to estimate level of support (global context)
% - has 695 input claims, and 16,636 verified (i.e. fact check) claims
% \citep{vo_lee_facts} % Where Are the Facts? Searching for Fact-checked Information to Alleviate the Spread of Fake News
% - *uses entire article
% - *novelty, elmo glove and euclidean distance for feature extraction in CNN
% - \textbf{does exactly our task}
% - used both Politifact and Snopes (dataset derived from these)
% - both text and image (if available) used for ranking
% - text expanded with OCR if available
% - used entire article (including images if present!), not just claim
% - initial re-ranking with BM25
% - after reranking
%     - GloVe embeddings used to find overlapping words (interaction matrix) by taking matmul cos sim (generates matrix of only 1s, or not 1s) (lets call this matrix S)
%     - ELMo embeddings create contextual word embeddings (why? raw glove encodings will show cossim of 1, even if context is different. Also, ELMo can capture context even through typos) (lets call this matrix C)
%     - attention matrix using euclidean distance on matrix S (A)
%     - S and A and C and (S-C) stacked and fed into CNN for feature extraction
%         - for images, ResNet is applied
%     \begin{figure}
%       \includegraphics[width=\linewidth]{images/vo_lee_fact_matrices.png}
%       \caption{matrices S (3), A (5), C (6)}
%       \label{fig:vo_lee_facts_matrices}
%     \end{figure}
% \citep{Sheng_2021} % Article Reranking by Memory-Enhanced Key Sentence Matching for Detecting Previously Fact-Checked Claims
% - *novelty
% - proposes novel re-ranked, leverages information about fact check articles
%     - events, semantical or lexical (claims are often quoted to describe the checked events, providing lexical information besides semantics)
%     - pattern information
%     - The reranker identifies key sentences per article using claim- and pattern-sentence relevance, and then integrates information from the claim, key sentences, and patterns for article-level relevance prediction
%     - This is quite a complex pipeline with a lot of different architectures and methodologies, summed up it is as below:
%         - 1) fine-tuned transformer (guided by ROUGE score to introduce lexical knowledge, i.e. RougeGuidedTransformer), captures semantic and lexical information, and generates score for a claim-sentence score (\texttt{for sentence in article})
%         - 2) trained Pattern Memory Bank (imagine as a web of possible article-sentence patterns) is used with K nearest Neighbors to obtain pattern-sentence scores
%         - 3) then, identifies top $k_{2}$ key sentences (from the article) by combining scores of previous two points
%         - 4) then, multi layer transformer models interaction with given query, given sentence, and nearest memory vector (from PMB, for each key sentence)
%         - 5) finally, score weighted aggregation is performed on output of (4) is performed for final result

% - “We propose a novel reranker MTM for factchecked claim detection, which can better identify key sentences in fact-checking articles by exploiting their characteristics. 
% • We design ROUGE-guided Transformer to combine lexical and semantic information and propose a memory mechanism to capture and exploit common patterns in fact-checking articles. 
% • Experiments on two real-world datasets show that MTM outperforms existing methods. Further human evaluation and case studies prove that our model finds key sentences as good explanations. 
% • We built the first Chinese dataset for factchecked claim detection with fact-checking articles from diverse sources.” ([Sheng et al., 2021, p. 5469](zotero://select/groups/4620027/items/A463XH47)) ([pdf](zotero://open-pdf/groups/4620027/items/58SJ4DVY?page=2&annotation=PSXTFFT9))
% \citep{mansour_did_2022}, % Did I See It Before? Detecting Previously-Checked Claims over Twitter
% - *standard
% - used CheckThatLab dataset
% - standard 3 process pipeline: 
%     - preprocessing, got URLs out of tweets with Twitter API, Meta Reverse Image Search API to perform reverse image search for pictures and videos and get a short description
%     - initial retrieval, quite a few including: Jelinek Mercer (JM), smoothing, RM3, DPH, PyTerrir was used in the end (indexing and retrieval)
%     - reranking
% - 
% - \textbf{does exactly our task}
% \citep{bhatnagar_abstractive_summarization_2022} % Harnessing Abstractive Summarization for Fact-Checked Claim Detection
% - *novelty of abstractive summairzation
% - using abstractive summarization on the POST (twitter). This is the first paper that seems to do this
% - Main contributions:
%     - 1. Workflow
%     - 2. Dataset ('Indian Context')
%     - 3. Fine-tuned Model
%     - 4. Experimental Analysis (Both statistical and qualitative of (of summaries)
% \citep{adler_realtime} % Real-time Claim Detection from News Articles and Retrieval of Semantically-Similar Factchecks
% - *standard
% - "fact checked claim detection", but uses quora question dataset
% - uses various embeddings technique with clustering (DBSCan clustering method to find optimal parameters)
% - the paper seems a bit sloppy and unprofessional, am willing to disregard it even though it falls into our task category
% - standard pipeline with embeddings
% - actually, this is just textual similarity
% \citep{crowdchecked_2022} % CrowdChecked: Detecting Previously Fact-Checked Claims in Social Media
% - *standard
% - provides strong overview for this task, mentions methods of baselines (CLEF namely)
% - large scale dataset
% - 330k twitter posts
% - slightly less FCs than SNOPES
% - we have more social medias
% - we have multiple languages (they specifically only crawled for English) - important to assess textual patterns across multilingual borders
% - more fact checks from different organization
% - we have less confirmed pairs but they are 100\% verified and confirmed, theirs are only estimates

% \citep{you_attributed_2020} % Attributed Multi-Relational Attention Network for Fact-checking URL Recommendation
% - *novelty, doesnt even look at text
% - "At the high level, AMRAN is composed of two modules as shown in Figure 3: (i) a convolutional spatial attention network (CSAN ) and (ii) a heterogeneous graph attention network (HGAN )."
% - does not focus on text, instead, contextual information regarding URLS and SMP

% \citep{jiang_categorising_2021} % Categorising Fine-to-Coarse Grained Misinformation: An Empirical Study of the COVID-19 Infodemic
% - *full post
% - "An information retrieval experiment to retrieve COVID-19 tweets that are related to the IFCN fact-checked misinformation.
% The fact-checked misinformation claims are used as the queries to extract tweets with topics that are similar to the
% misinformation."
% - "A manually annotated fine-grained COVID-19 misinformation Twitter dataset with 8 categories that are suitable for
% training machine learning models to automatically detect misinformation and social behaviours related to COVID-19
% misinformation."
% - mainly only covid
% - only 90 fact check claims (not even full article), with claim extraction
% - 1800 manually annotated tweets

% \citep{wang_relevant_2018} % Relevant Document Discovery for Fact-Checking Articles
% - *standard
% - only uses claims, not full social media posts
% - Three stages:
%     1. Retrieve candidate documents based on various features in the fact-checking article
%     2. Apply relevance classifier to filter away documents that do not address the claim
%     3. Apply language feature based classifier to distinguish documents with different stances towards the claim.
% - does it in reverse (query is article, result is social media post/document/claim)
% - Dataset used:
%     - ClaimReview JSON Markup (with filtering)

% ======================================================
% =========== IMPORTANT NOTES ==========================
% ======================================================

% \paragraph{Shortcoming in Current Literature}
% Important Shortcomings currently in Literature! There won't be a seperate piece of text in this section, but just keeping track of some of the main points to outline throughout literature review!!
% - no cross-lingual exploration done for fake news detection combating low-resource availability (of datasets, but also affects strength of methodology)
% - no one investigated as detailed of a pipeline as us (translation, preprocessing, sliding window, text concatenation, rank aggregation, and more). 
% - People typically perform little to none pre-processing in a naive fashion. No one investigated it as much as us.
% - \textbf{no one has as extensive of a database as us (both SMP and FC)} - This is really key in assessing broader connections, patterns, and semantic elements in a multingual setting, which no has done \textit{nearly} as extensively as us.
% - topic analysis (no one has investigated this!!!)
% - language analysis (no one has investigated this!!!)
%     - code switching analysis! 
%     - different methods results in terms of languages (Matus 18th oct graphs on doc displays this very nicely)
% - timeline analysis 
% - only limited dataset
% - re-ranking performed only on top 100 results (usually). However, we calculate cosine similarity efficiently for all pairs. This gives better insight into the performance of LM embeddings for previously fact checked claim detection as they are being assessed on a wider variety of pairs, and not just those with phenomenal scores from BM25
% - anything more?
% - the claim matching is often defines as a (binary) classification problem. this is however unpractical if we wish to search in the fact checks. performing 100ks of classifications is too expensive. e.g. https://aclanthology.org/2022.findings-naacl


% \paragraph{Shortcomings in Our Paper}
% - no claim extraction/top claim extraction/abstractive summarization used on tweets (or potentially on FC claim/title as well)
% - no supervised (perhaps even unsupervised/heuristic based) re-ranking used

% TODO: Decide if the dataset section(s) should be seperate from the literature review, or mentioned throughout in their respective section


% Put all of this information into a single table, containing all relevant information
% This includes: size, input fields, verified claim fields, no. of verified pairs, available metadata, amount of languages and their entry counts, (anything else?)
% \paragraph{Datasets for Previously Fact Checked Claim Detection (Input - Claim Format}
% - note, these are all tiny in comparison to our dataset :))
% - \citep{shaar-etal-2020-known} % That is a Known Lie: Detecting Previously Fact-Checked Claims
% - That is a Known Lie
% - 2 datasets: 1) Politifact, 2) Snopes, both found on here: https://github.com/sshaar/That-is-a-Known-Lie
%     - 1) Politifact: 
%     - 2) Snopes:
% - \citep{claimsKG_2019} % ClaimsKG: A Knowledge Graph of Fact-Checked Claims
% - ClaimsKG, is only claims

% - \citep{ashkan_kazemi_2021}
% - Claim Detection and Matching for Indian Languages (contains also English)
% - published on Zenodo here: https://zenodo.org/record/4890950\#.Y0WZyXbMI2w
% - "We construct a novel dataset of WhatsApp tipline and public group messages alongside fact-checked claims that are first annotated for containing “claim-like statements” and then matched with potentially similar items and annotated for claim matching"

% - \citep{hossain-etal-2020-covidlies} % COVIDLIES: Detecting COVID-19 Misinformation on Social Media
% - COVID19Lies
% - two tasks covered here:
%     - (i) "retrieval of misconceptions relevant to posts being checked for veracity" (sets up part 2)
%     - (ii) stance detection to identify whether the posts Agree, Disagree, or express No Stance towards the retrieved misconceptions (almost nearly our task, but we dont use labels, we do absolute rankings, a harder problem)
% - 6,761 expert-annotated tweets mapped to 86 different pieces of COVID-19 related misinformation and containing stance labels (stance of tweets towards the misinformation)
% misconceptions 
% - extracted from a Wikipedia article about COVID-19 misinformation
% tweets 
% - from COVID-19-related tweets identified in a previous work they select 100 most similar tweets for each misconception (using BERTscore) and then label them manually
% 85.02\% No stance, 9.91\% Agree, 5.07\% Disagree
% - small and unbalanced dataset...

% - \citep{Sheng_2021} % Article Reranking by Memory-Enhanced Key Sentence Matching for Detecting Previously Fact-Checked Claims
% - MTM (Twitter and Weibo)
% - For Chinese dataset, from paper:
%     - "To validate the effectiveness of our method, we built the first Chinese dataset for this task with 11,934 claims collected from Chinese Weibo3 and 27,505 fact-checking articles from multiple sources. 39,178 claim-article pairs are annotated as relevant."
% - For English Dataset
%     - Twitter Dataset format unified with
%     - Weibo dataset
%     - both mentioned here: https://github.com/ICTMCG/MTM
%     - Basically just combinations of Snopes and Politifact.


